The Secret Life of CVEs

The Common Vulnerabilities and Exposures (CVEs) system is a reference method for documenting publicly known information security weaknesses and exposures. This paper presents a study of the lifetime of CVEs in software projects and the risk factors affecting their existence. The study uses survival analysis to examine how features of programming languages, projects, and CVEs themselves impact the lifetime of CVEs. We suggest avenues for future research to investigate the effect of various factors on the resolution of vulnerabilities.

==> tools/table.tex <==

\renewcommand\thetable{1.4}

\begin{table}[htb]

\caption{Languages coexisting in CVE lifetime}
\end{table}

\begin{tabular}{lr@{\hspace{1ex}}rll}
  \toprule
  Variable             & \multicolumn{2}{l}{N(\%)} & $\tilde{Y}_{\text{med}}$    & $D_{xy}$    \\
  \midrule
  %%
  %% most common language
  \rowcolor[HTML]{C0C0C0}
  Type checking  & 62866 &   (100\%)   &  34.0  & $-0.05$ \\
  static         & 28065 & (44.64\%)   & 44.0  &  \\
  dynamic        & 34801 & (55.36\%)   & 27.0   &   \\
  %%
  \rowcolor[HTML]{C0C0C0}
  Type safety  & 62866 &   (100\%) & 34.0 & $+0.04$  \\
  strong       & 34357 & (54.65\%) & 29.0 &     \\
  weak         & 28509 & (45.35\%) & 42.0 &  \\
  %%
  \rowcolor[HTML]{C0C0C0}
  Memory model  & 62866 &   (100\%) & 34.0 & $+0.07$  \\
  managed       & 42269 & (67.24\%) & 27.0 & \\
  non managed   & 20597 & (32.76\%) & 56.0 & \\
  %%
  %% CVE metadata
  % access, impact etc
  % \rowcolor[HTML]{C0C0C0}
  % Access Authentication & 62646 & (99.65\%) & 34.0 & $-0.02$ \\
  % NONE     &  57560 & (91.56\%) &    35.0 & \\
  % SINGLE   &   5065 &  (8.06\%) &    22.0 & \\
  % MULTIPLE &     21 &  (0.03\%) &    20.0 & \\
  %%
  \rowcolor[HTML]{C0C0C0}
  Access complexity (AC) & 62646 & (99.65\%) & 34.0 & $-0.04$  \\
  LOW      &  35933 & (57.16\%) &    39.0 & \\
  MEDIUM   &  24081 & (38.31\%) &    31.0 & \\
  HIGH     &   2632 &  (4.19\%) &    18.5 & \\
  %%
  \rowcolor[HTML]{C0C0C0}
  Access vector (AV) &  62646 & (99.65\%) &    34.0 & $-0.07$ \\
  LOCAL         &  12897 & (20.52\%) &    67.0 & \\
  ADJACENT      &   1108 &  (1.76\%) &    35.0 & \\
  NETWORK       &  48641 & (77.37\%) &    28.0 &  \\
  %%
  \rowcolor[HTML]{C0C0C0}
  Availability impact (A) & 62646 & (99.65\%) & 34.0 & $+0.02$ \\
  NONE        &  14991 & (23.85\%) & 30.0 & \\
  PARTIAL     &  32005 & (50.91\%) & 35.0	 & \\
  COMPLETE    &  15650 & (24.89\%) & 37.0 &  \\
  %%
  \rowcolor[HTML]{C0C0C0}
  Confidentiality impact (C) & 62646 & (99.65\%) & 34.0 & $-0.02$ \\
  NONE     &  23966 & (38.12\%) &    39.0 & \\
  PARTIAL  &  27527 & (43.79\%) &    31.0 & \\
  COMPLETE &  11153 & (17.74\%) &    31.0 & \\
  %%
  \rowcolor[HTML]{C0C0C0}
  Integrity impact (I) & 62646 & (99.65\%) & 34.0 & $-0.05$ \\
  NONE      &  26236 & (41.73\%) &    44.0 & \\
  PARTIAL   &  25710 & (40.90\%) &    28.0	 & \\
  COMPLETE  &  10700 & (17.03\%) &    29.0 & \\
  %%
  % \rowcolor[HTML]{C0C0C0}
  % CVSS v2.0 Ratings &  62646 & (99.65\%) &  34.0 & $-0.02$ \\
  % Low               &   5569 &  (8.86\%) &  51.0 & \\
  % Medium            &  38315 & (60.95\%) &  34.0	 & \\
  % High              &  18762 & (29.84\%) &  31.0 & \\
  %%
  \rowcolor[HTML]{C0C0C0}
  CVSS v3.1 Ratings &  62646 & (99.65\%) &  34.0 & $-0.03$ \\
  None+Low          &   5569 &  (8.89\%) &  51.0 & \\
  Medium            &  38315 & (61.16\%) &  34.0 & \\
  High              &  13542 & (21.62\%) &  35.0 & \\
  Critical          &   5220 &  (8.33\%) &  21.0 & \\
  %%
  %% project metadata
  %%
  \rowcolor[HTML]{C0C0C0}
  NumAuthors (3 bins)  & 62813 & (99.92\%) & 34.0   & $+0.10$ \\
  $[1, 100)$           & 27098 & (43.14\%) & 24.0	&  \\
  $[100, 1000)$        & 27098 & (28.71\%) & 28.0	& \\
  $[1000, \infty)$     & 17680 & (28.15\%) & 68.0	& \\
  %%
  \rowcolor[HTML]{C0C0C0}
  NumCore (3 bins)     & 62813 & (99.92\%) & 34.0   & $+0.09$ \\
  $[1, 5)$             & 16872 & (26.86\%) & 29.0	&  \\
  $[5, 50)$            & 23188 & (36.92\%) & 20.0	& \\
  $[50, \infty)$       & 22753 & (36.22\%) & 61.0	& \\
  %%
  \rowcolor[HTML]{C0C0C0}
  NumFiles (3 bins)    & 62866 & (100\%)   & 34.0 & $+0.05$ \\
  $[1, 10^4)$          & 21171 & (33.68\%) & 25.0 &  \\
  $[10^4, 10^5)$       & 19791 & (31.48\%) & 37.0 & \\
  $[10^5, \infty)$     & 21904 & (34.84\%) & 41.0 & \\
  %%
  \rowcolor[HTML]{C0C0C0}
  ActiveMon [\%] (3 bins) & 62866 & (100\%)   & 34.0 & $-0.10$ \\
  $[0.0,  50.0)$          & 15692 & (24.96\%) & 64.0 &  \\
  $[50.0, 85.0)$          & 18399 & (29.27\%) & 32.0 & \\
  $[85.0, 100.0]$         & 28775 & (45.77\%) & 25.0 & \\
\bottomrule
\end{tabular}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "table_preview"
%%% End:


==> tools/table_preview.tex <==
\input{default_packages}

\begin{document}

\input{table}

\end{document}

